DiffFacto: Controllable Part-Based 3D Point Cloud Generation with Cross Diffusion

While the community of 3D point cloud generation has witnessed a big growth in recent years, there still lacks an effective way to enable intuitive user control in the generation process, hence limiting the general utility of such methods. Since an intuitive way of decomposing a shape is through its parts, we propose to tackle the task of controllable part-based point cloud generation. We introduce DiffFacto, a novel probabilistic generative model that learns the distribution of shapes with part-level control. We propose a factorization that models independent part style and part configuration distributions and presents a novel cross-diffusion network that enables us to generate coherent and plausible shapes under our proposed factorization. Experiments show that our method is able to generate novel shapes with multiple axes of control. It achieves state-of-the-art part-level generation quality and generates plausible and coherent shapes while enabling various downstream editing applications such as shape interpolation, mixing, and transformation editing. Project website: https://difffacto.github.io/

==> sections/8-Acknowledgment.tex <==
\section{Acknowledgment}
This work is supported by ARL grant W911NF-21-2-0104, a Vannevar Bush Faculty Fellowship, the Natural Science Foundation of China (Project No. 62220106003), Tsinghua-Tencent Joint Laboratory for Internet Innovation Technology, and the Natural Sciences and Engineering Research Council of Canada. We very much appreciate Congyue Deng for her helpful discussion at the early stage of this project. We are also grateful for the advice and help from Colton Stearns and Davis Rempe.


==> tables/ablation-cnf.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{9pt}
\begin{tabular}{l|ccc}
    \toprule
 & MMD-P ($\downarrow$) & COV-P ($\uparrow$) & 1NNA \\
\midrule
VAE & \red{TODO} & \red{TODO} & \red{TODO} \\
CNF (Ours) & \red{TODO} & \red{TODO} & \red{TODO}\\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation on Part Stylizer.} Individual-part level metrics ablating our part stylizer (MMD-P $\times 10^{-4}$).}
\label{tab:ablation-cnf}
\end{table}

==> tables/score-recon.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{6.5pt}
\begin{tabular}{l|cccc}
\toprule
& Chair& Airplane  &Lamp & Car\\ 
\midrule=7cm
reg. diffusion  & 5.30 & 2.27 & 8.33 & 7.69\\
reg. diffusion w/ parts & 4.39  & 1.70  & 5.55  & 7.01\\ 
\midrule
Ours w/o gen.ker.& \underline{3.76} & \underline{1.46}  & \underline{3.82}  & \underline{6.56}\\
\textbf{\methodname} (Ours) & \textbf{3.71} & \textbf{1.41}  &\textbf{3.48} & \textbf{6.54}\\ 
\bottomrule
\end{tabular}
\caption{ \textbf{Reconstruction Score}. Reconstruction score on the point cloud autoencoding task  (CD $\times 10^{-4}$).}
\vspace*{-0.5\baselineskip}
\label{tab:score-recon}
\end{table}
